Universal energy-speed-accuracy trade-offs in driven nonequilibrium systems

Physical systems driven away from equilibrium by an external controller dissipate heat to the environment; the excess entropy production in the thermal reservoir can be interpreted as a "cost" to transform the system in a finite time. The connection between measure theoretic optimal transport and dissipative nonequilibrium dynamics provides a language for quantifying this cost and has resulted in a collection of "thermodynamic speed limits", which argue that the minimum dissipation of a transformation between two probability distributions is directly proportional to the rate of driving. Thermodynamic speed limits rely on the assumption that the target probability distribution is perfectly realized, which is almost never the case in experiments or numerical simulations. Here, we address the ubiquitous situation in which the external controller is imperfect. As a consequence, we obtain a lower bound for the dissipated work in generic nonequilibrium control problems that 1) is asymptotically tight and 2) matches the thermodynamic speed limit in the case of optimal driving. We illustrate these bounds on analytically solvable examples and also develop a strategy for optimizing minimally dissipative protocols based on optimal transport flow matching, a generative machine learning technique. This latter approach ensures the scalability of both the theoretical and computational framework we put forth. Crucially, we demonstrate that we can compute the terms in our bound numerically using efficient algorithms from the computational optimal transport literature and that the protocols that we learn saturate the bound.

==> preamble.tex <==
\usepackage[english]{babel}

\makeatletter
% A change to a babel macro
\def\bbl@set@language#1{%
  \edef\languagename{%
    \ifnum\escapechar=\expandafter`\string#1\@empty
    \else\string#1\@empty\fi}%
  %%%% ADDITION
  \@ifundefined{babel@language@alias@\languagename}{}{%
    \edef\languagename{\@nameuse{babel@language@alias@\languagename}}%
  }%
  %%%% END ADDITION
  \select@language{\languagename}%
  \expandafter\ifx\csname date\languagename\endcsname\relax\else
    \if@filesw
      \protected@write\@auxout{}{\string\select@language{\languagename}}%
      \bbl@for\bbl@tempa\BabelContentsFiles{%
        \addtocontents{\bbl@tempa}{\xstring\select@language{\languagename}}}%
      \bbl@usehooks{write}{}%
    \fi
  \fi}
% The user interface
\newcommand{\DeclareLanguageAlias}[2]{%
  \global\@namedef{babel@language@alias@#1}{#2}%
}
\makeatother

\DeclareLanguageAlias{en}{english}

\DeclareLanguageAlias{en}{english}


\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\DeclareUnicodeCharacter{3B1}{\ensuremath{\alpha}}
\algrenewcommand{\algorithmiccomment}[1]{$\vartriangleright$ #1}
\algrenewcommand{\algorithmicreturn}{\textbf{Return: }}
\algnewcommand\algorithmicinput{\textbf{Input: }}
\algnewcommand\Input{\State \algorithmicinput}

\usepackage{amsmath, amssymb}
\usepackage[x12names, rgb, html]{xcolor}

\definecolor{red}{HTML}{f54b1a}
\definecolor{pink}{HTML}{d19eb1}
\definecolor{orange}{HTML}{d3772e}
\definecolor{yellow}{HTML}{ebe85d}
\definecolor{green}{HTML}{0f6852}
\definecolor{lightblue}{HTML}{01abe9}
\definecolor{darkblue}{HTML}{1b346c}
\definecolor{tan}{HTML}{e5c39e}
\definecolor{darktan}{HTML}{af9e73}
\definecolor{grey}{HTML}{c3ced0}
\definecolor{darkgrey}{HTML}{9dadc4}
\definecolor{black}{HTML}{110d1b}
\definecolor{white}{HTML}{f1f8f1}


\usepackage{hyperref}
\hypersetup{
  colorlinks = true,
  linkcolor = red,
  citecolor = darkblue,
  urlcolor = lightblue
}

\usepackage{caption}
\captionsetup{justification=raggedright,singlelinecheck=false}
%\usepackage[margin=1in]{geometry}

\newcommand{\grant}[1]{\marginpar{\huge \textcolor{green}{$\star$}} \textcolor{green}{GMR: #1}}
\newcommand{\jeremie}[1]{\marginpar{\huge \textcolor{red}{$\star$}} \textcolor{red}{JK: #1}}
\renewcommand{\thefootnote}{$\star$}


%\usepackage{ebgaramond}
%\usepackage[cmintegrals,cmbraces]{newtxmath}
%\usepackage{ebgaramond-maths}
% \usepackage{fontspec}
% \setmainfont[]{ebgaramond}
% \setmainfont[
%     Path = theme/,
%     Ligatures=TeX,
%     UprightFont = et-book-roman-old-style-figures,
%     ItalicFont = et-book-display-italic-old-style-figures,
%     BoldItalicFont = et-book-semi-bold-old-style-figures,
%     BoldFont = et-book-bold-line-figures
%   ]{}

\usepackage{graphicx}
\graphicspath{{figs/}}


\newcommand{\diff}[3]{\frac{\partial^{#3}#1}{\partial #2^{#3}}}
\newcommand{\Diff}[3]{\frac{d^{#3}#1}{d #2^{#3}}}

\newcommand{\bfm}[1]{\mathchoice {\mbox{\boldmath$\displaystyle#1$}}
    {\mbox{\boldmath$\textstyle#1$}}
    {\mbox{\boldmath$\scriptstyle#1$}}
    {\mbox{\boldmath$\scriptscriptstyle#1$}}}

\def\d{\mathsf{d}} 


\def\rhoeq{\varrho_{\rm eq}}
\def\nb{\boldsymbol{n}}
\def\rhob{\boldsymbol{\rho}}
\def\varrhob{\boldsymbol{\varrho}}
\def\thetab{\boldsymbol{\theta}}
\def\varthetab{\boldsymbol{\vartheta}}
\def\etab{\boldsymbol{\eta}}
\def\mub{\boldsymbol{\mu}}
\def\xib{\boldsymbol{\xi}}
\def\ab{\boldsymbol{a}}
\def\bb{\boldsymbol{b}}
\def\cb{\boldsymbol{c}}
\def\qb{\boldsymbol{q}}
\def\pb{\boldsymbol{p}}
\def\Ab{\boldsymbol{A}}
\def\Qb{\boldsymbol{Q}}
\def\Jb{\boldsymbol{J}}
\def\kb{\boldsymbol{k}}
\def\rb{\boldsymbol{r}}
\def\vb{\boldsymbol{v}}
\def\wb{\boldsymbol{w}}
\def\xb{\boldsymbol{x}}
\def\yb{\boldsymbol{y}}
\def\zb{\boldsymbol{z}}

\def\Mb{\boldsymbol{M}}
\def\Tb{\boldsymbol{T}}
\def\Xb{\boldsymbol{X}}
\def\Zb{\boldsymbol{Z}}
\def\Xbu{\boldsymbol{X}^{u}}
\def\Xbc{\boldsymbol{X}^{c}}
\def\Wb{\boldsymbol{W}}

\def\Xu{X^{u}}

\def\grad{\nabla}
\def\div{\nabla \cdot}
\def\lap{\Delta}

\def\sscr{\scriptscriptstyle} \def\sp{\vspace{2mm}}

\def\lap{\Delta}
\def\eps{\varepsilon}

\def\RR{\mathbb{R}} \def\NN{\mathbb{N}} \def\ZZ{\mathbb{Z}}
\def\EE{\mathbb{E}}\def\PP{\mathbb{P}}

\newcommand{\ddt}{\frac{\partial}{\partial t}}
\newcommand{\ddx}{\frac{\partial}{\partial x}}
\newcommand{\avg}[1]{\mathbb{E}\left[ #1 \right]}

\def\<{\langle} \def\>{\rangle}

\DeclareRobustCommand{\ran}{\operatorname*{ran}}
\DeclareRobustCommand{\supp}{\operatorname*{supp}}
\DeclareRobustCommand{\argmin}{\operatorname*{argmin}}
\DeclareRobustCommand{\sign}{\operatorname*{sign}}

